Distributed Deep Learning for Modulation Classification in 6G Cell-Free Wireless Networks

In the evolution of 6th Generation (6G) technology, the emergence of cell-free networking presents a paradigm shift, revolutionizing user experiences within densely deployed networks where distributed access points collaborate. However, the integration of intelligent mechanisms is crucial for optimizing the efficiency, scalability, and adaptability of these 6G cell-free networks. One application aiming to optimize spectrum usage is Automatic Modulation Classification (AMC), a vital component for classifying and dynamically adjusting modulation schemes. This paper explores different distributed solutions for AMC in cell-free networks, addressing the training, computational complexity, and accuracy of two practical approaches. The first approach addresses scenarios where signal sharing is not feasible due to privacy concerns or fronthaul limitations. Our findings reveal that maintaining comparable accuracy is remarkably achievable, yet it comes with an increase in computational demand. The second approach considers a central model and multiple distributed models collaboratively classifying the modulation. This hybrid model leverages diversity gain through signal combining and requires synchronization and signal sharing. The hybrid model demonstrates superior performance, achieving a 2.5% improvement in accuracy with equivalent total computational load. Notably, the hybrid model distributes the computational load across multiple devices, resulting in a lower individual computational load.

==> SotA.tex <==
\section{Related Work}
% What is offset, skew and drift?
The local notion of time in most sensor-nodes is generated by the oscillator, it provides clock ticks. The literature differentiate three different terms when discussing the non-ideal behaviour of clocks: \textit{Offset} which is the delay between two clocks, when this value is zero, both clocks are perfectly synchronized. \textit{Skew} is the difference between the frequencies of the clocks. \textit{Drift} refers to small variations on the skew, usually as consequence of environmental changes such as Temperature \cite{basics}.    


% How to compensate for offset
    % Why not GPS 
Several papers presented methods to eliminate the clock offset in large-scale networks, passively by using reference signals \cite{airsync} or actively by propagating synchronization-signals over the network \cite{PulseSync}. However, these methods fail to meet the strict synchronization requirements of distributed networks. Currently, GPS synchronization is a widely adopted method for providing accurate synchronization over large distances. Nevertheless, GPS receivers add a non-negligible cost to each node and are prone to spoofing \cite{spoofing}.



% How to compensate for skew and drift
State-of-the-art methods focusing on the compensation of the clock skew and drift are usually conducted for wireless sensor networks with limited RF-capabilities. While some works consider compensation methods based on linear programming and multi-cast \cite{linearprogramming}, most research reports are centered around temperature-assisted methods \cite{linearprogramming,Temp_assisted,Temperature}. This arises from the strong correlation between the working-temperature and the oscillator-frequency. 

Obtaining a good temperature-frequency model requires accurate measurements of the oscillator frequency, which can be challenging to obtain. To this end, some research considers a static model by which the temperature-frequency model is approximated using a second order or third order polynomial \cite{Temp_assisted}. The weights for the second and third order polynomial are estimated using a priory measurements. More recent work focuses on a dynamic model based on lookup-tables and interpolation between known temperature-frequency pairs\cite{nB-iot}. However, most research in this domain targets low-end oscillators which have a more outspoken temperature-frequency correlation compared to the high-end oscillators considered in this work. The required accuracy of the models fail to meet the required accuracy considered in this work. To the best of the authors’ knowledge, LSTM and online-LSTM have not been considered for modeling the temperature-frequency behavior the oscillator. 

%\sofie{State of the art on the use of other signals than GPS, e.g., LTE or ADS-B or....?}

%% How do they estimate the ppm in state of the art? 
